A New Super-Resolution Measurement of Perceptual Quality and Fidelity

Super-resolution results are usually measured by full-reference image quality metrics or human rating scores. However, these evaluation methods are general image quality measurement, and do not account for the nature of the super-resolution problem. In this work, we analyze the evaluation problem based on the one-to-many mapping nature of super-resolution, and propose a novel distribution-based metric for super-resolution. Starting from the distribution distance, we derive the proposed metric to make it accessible and easy to compute. Through a human subject study on super-resolution, we show that the proposed metric is highly correlated with the human perceptual quality, and better than most existing metrics. Moreover, the proposed metric has a higher correlation with the fidelity measure compared to the perception-based metrics. To understand the properties of the proposed metric, we conduct extensive evaluation in terms of its design choices, and show that the metric is robust to its design choices. Finally, we show that the metric can be used to train super-resolution networks for better perceptual quality.

==> Fourier.tex <==
% \section{Fourier Analysis on Deep Neural Network}

% The training process of deep neural network plays an important role in interpretation of deep neural network. In paper\cite{arpit2017closer}, the deep neural networks tend to learn simple pattern first and then complicated pattern. In frequency domain, the paper\cite{xu2018training}\cite{xu2019frequency} shows that deep neural network converages at low frequency first and then high frequency. 

% There are several methods that analyze how deep neural network works. One of method is to evaluate model on validation/test dataset which shows the generation error. In a training step, if some parts of validation datasets has better performance than the other part, it reflects that deep neural networks prefer to learn this part of dataset. The paper\cite{arpit2017closer} uses this evaluation method. Another method is back to the training process such as analyzing the norm of gradient of deep neural network which reflects converage speed. If the norm of gradient is large, for a fix step-size, the update speed for the each iteration is faster than small gradient. 

% In this report, we focus on analyze the deep neural network on training dataset at training stage in frequency domain. The original loss function for a deep neural network is $L_{s} = \frac{1}{N}\sum_{x}(f(x) - T(x))^_{2}$. According to Parseval's theorem, the loss function could be expressed in frequency domain, which is $L_{f} = \frac{1}{N} \sum_{\gamma}|F(f)(\gamma) - F(T)(\gamma)|^{2}$. Here, the Fourier transform of the deep neural network is $F(f) = \sum_{j = 0}^{n-1} y_{j}exp(-2\pi i x_{j}k)$. Therefore, instead of analyzing how each sample contributes to loss function and training process, in frequency domain, we focus on how each frequency contributes to them. 

% In subsection1.1, we shows the relationship between norm of gradient and frequency. In subsection1.2, we shows how we apply the analysis on super resolution problem. 

% \subsection{Relationship between norm of gradient and frequency}

% According to the paper\cite{xu2018training}, at frequency $k$, the Fourier transform of target function is $F[f](k)$, the Fourier transform of DNN output is $F(T)(k)$. Thus, we define the distance between DNN outputs and target at frequency $k$ is $D(k)$
% $$D(k) = F[f](k) - F(T)(k) = A(k)\exp(i\theta(k))$$
% we consider the $\delta(x) = tanh(x)$ as activation function, expressed as $F(T)(k) = \sum^{N}_{j}a_j\delta(w_{j}x+b_{j})$. The gradient of loss function is 
% $$|\frac{\partial L(k)}{\partial \theta_{jl}}| = A(k)\exp(-|\frac{\pi k}{2w_{j}}|)G_{jl}(\theta_{l}, k)$$
% Here, $\theta_{j} = \{\theta_{j0}, \theta_{j1}, \theta_{j2}\} \overset{\Delta}{=} \{w_{j}, b_{j}, a_{j}\}$. The influence of $G_{jl}(\theta_{l}, k)$ part is small and could be ignored. Therefore, the norm of gradient is mainly determined by 
% $$|\frac{\partial L(k)}{\partial \theta_{jl}}| = A(k)\exp(-|\frac{\pi k}{2w_{j}}|)$$.

% Based on this formulation, it shows that at early stage, the gradient at small frequency is larger than the gradient at large frequency. In addition, it exists the situation that the gradient at different frequency is same. Both of this analysis shows that the DNN tends to converage at low frequency first and then converage at high frequency. 

% \subsection{Applying the Fourier Analysis on Super Resolution problem}

% In formulation $F(f) = \sum_{j = 0}^{n-1} y_{j}exp(-2\pi i x_{j}k)$, we need to determine the input $x$, the corresponding output $y$, as well as $k = |k|\Vec{p}$. In the paper\cite{xu2019frequency}, the target problem is classification problem on MNIST dataset. The input is vectorized number image. The output is a binary classification result determined by whether the output label belongs to one of specific categories. The direction of $k$ is the first principle component of input images.   

% Correspondingly, in super resolution problem, the input is low resolution image patch. The output is corresponding high resolution image patch. The area of output patch is depended on the receptive field. More specifically, we just consider one pixel point as output in this report. The direction of $k$ is also the direction of first principle component of input image patches. However, there are two possible format for output pixel. We will discuss it in next section.



% %-------------------------------------------------------------------------
% \section{Different Target Function}
% There are two possible target function for the formulation $F(f) = \sum_{j = 0}^{n-1} y_{j}exp(-2\pi i x_{j}k)$. One is directly use pixel value as target output. The other is considered as a binary classification. We set the output as 1 if the the output image pixel value is equal to a specific pixel value. Otherwise, we set the output to 0. In next subsections, we will show that the second method works for super resolution problem while the first method meets some problem and our attempts.
% \subsection{Pixel Value as Target Output}

% We transfer the evaluation method on DNN model from paper\cite{xu2019frequency}. However, there are some problems. First of all, we will introduce some settings in that paper. And then we will shows what are the problems. 

% In paper\cite{xu2018training}, after getting the Fourier transform of ground truth and prediction on each epoch. They measure the the relative difference by $\Delta_{F} = \frac{|F[f](k) - F(T_{t})(k)|}{|F[f](k)|}$. Here $t$ is the step number, and $T_{t}$ means the DNN models at step $t$. In addition, in their experiment, they just choose the frequency peak for evaluation which shows straightforward result compared with all frequency range. 

% In our experiment, both the frequency peak and relative difference do not work. Our observations are:
% \begin{itemize}
% \item In all frequency range, at early step(nearly at first 20 steps), the DNN outputs is pretty close to ground truth in frequency domain. After the early step, the absolute difference is small. 
% \item For relative difference, due to the absolute difference at low frequency and high frequency is not obvious, it does not show the principle that relative difference at low difference is smaller than that at high frequency. Therefore, we observe that sometimes, at some frequency, the high frequency converages faster than low frequency which is conflict with our analysis.   
% \item Frequency Peak does show better representation ability than other frequency range.
% \end{itemize}

% All three observations shows that nearly all frequency converages at same speed. We hypothesis that if we use the area that have worse Reconstruction result, it will be possible to show the principle that DNN converages at low frequency first and then high frequency. However, the experiment does not show expected result.

% \subsection{Binary Classification as Target Output}

% We change the output setting to binary classification case. In this experiment, we set region whose pixel value is equal to 128 to 1. Otherwise, the region is set to 0. We have the observation that the DNN converages at low frequency first and then high frequency. However, we have another observation that even at last epoch, there is still a gap between the prediction result and ground truth. 

% One of the explanation is that the super resolution problem is an inverse problem which one input could have several mappings to outputs. However, in experiment setting, we just choose one of the results as the ground truth. 

% \section{Evaluation on different models}

% After determining the classification as the target function, in this section, we first reproduces the PSNR result on different models. Then we analyze the different models on frequency domain. In this report, we compare eight different models. They are SRCNN\cite{dong2016image}, VDSR\cite{kim2016accurate}, LapSRN\cite{lai2018fast}, DDBPN\cite{haris2018deep}, EDSR\cite{lim2017enhanced}, RCAN\cite{Zhang_2018_ECCV}, ESRGAN\cite{Wang_2018_ECCV_Workshops}, PESR\cite{Vu_2018_ECCV_Workshops}. Especially, for ESRGAN and PESR model, we get results separately on PSNR based and GAN based training strategy.  

% \begin{table}
% \begin{center}
% \begin{tabular}{|1|c|c|}
% \hline
% Method & Set5 & Set14 \\
% \hline\hline\hline
% VDSR & 31.37 & 28.04 \\
% LapSRN & 31.62 & 28.22 \\
% DDBPN & 32.43 & 28.76\\
% EDSR & 32.50 & 28.81 \\
% RCAN & 32.65 & 28.85 \\
% ESRGAN(PSNR) & 32.72 & 28.96 \\
% ESRGAN(GAN) & 30.47 & 26.28 \\
% PESR(PSNR) & 32.47 & 28.79 \\
% PESR(GAN) & 28.80 & 25.93 \\
% \hline
% \end{tabular}
% \end{center}
% \caption{Reproduce results on different models}
% \end{table}

% It is clear to observe in table1 that deep residual network improves PSNR results a lot from 31 to 32. In addition, in a same model, training strategy on improving PSNR result shows better PSNR result compared with GAN based training strategy. However, the GAN based model at Fourier transform fits the ground truth better than PSNR based model. 

% In next section, we will explain the gap between these measurements. 

% \subsection{The Gap between Fourier distance and distribution distance}
% In this section, we will explore the gap between the Fourier distance and distribution distance. We will formulate the problem first and then show the proof.

% First, we define two sets of variables $X^{Est}, X^{Gt} \in \{0,1,...,254,255\}$. $D_X, D_{X^*}$ are the distribution of $X, X^*$, which are the prediction distribution and ground truth distribution. 
% According to the definition of the Fourier transform on non-uniform sampling, the formualtion is:
% $$F_{x_0}[X](\xi) = \frac{1}{N}\sum_{n}\mathbbm{1}(X_n = x_0) e^{-i\xi\vec{k}\cdot\vec{I_{n}}}$$
% For a fixed frequency $\xi$ and $t_0 = \vec{k}\cdot\vec{I}$, the Fourier distance for a pixel value $x_{0}$ is defined as 
% \begin{align*}
%     & FD_{x_{0}}[X, X^*| t_0= \vec{k}\cdot\vec{I}](\xi)  \\
%     =& |F_{x_{0}}[X| t_0](\xi) - F_{x_{0}}[X^{*}| t_0](\xi)| \\
%     = &\frac{1}{N} \left| \sum_{n, s.t.,\vec{k}\cdot\vec{I}_{n}=t_0} \mathbbm{1}(X_n = x_{0}) e^{-i\xi\vec{k}\cdot\vec{I}_{n}} - \sum_{n, s.t.,\vec{k}\cdot\vec{I}_{n}} \mathbbm{1}(X^{*}_n = x_{0}) e^{-i\xi\vec{k}\cdot\vec{I}_{n}} \right| \\ 
%     = &\frac{|e^{-i \xi t_0}|}{N}\left| \sum_{n, s.t.,\vec{k}\cdot\vec{I}_{n} = t_0}  \mathbbm{1}(X_n = x_{0})）  - \sum_{n, s.t.,\vec{k}\cdot\vec{I}_{n} = t_0} \mathbbm{1}(X^{*}_n = x_{0})）\right| \\
%     = &\frac{1}{N}\sum_{n, s.t.,\vec{k}\cdot\vec{I}_{n} = t_0} \left| \mathbbm{1}(X_n = x_{0})）  -  \mathbbm{1}(X^{*}_n = x_{0})）\right| \\
%     = &|P(X = x_0|t_0) - P(X^{*} = x_0|t_0)|
% \end{align*}

% \zhe{Consider a metric by averaging $|P(X = x_0|t_0) - P(X^{*} = x_0|t_0)|$, which corresponds to $\sum_{t_0} FD_{x_{0}}[X, X^*| t_0= \vec{k}\cdot\vec{I}](\xi)$.}

% \sheng{
% Now, the distribution metric works, which is:
% $$\text{Distribution Distance}(X, X^*) = \sum_{t_0}P(t_0)\sup_{x_0 \in \{0, 1, ..., 255\}}|P(X = x_0|t_0) - P(X^{*} = x_0|t_0)|$$

% What we know is that $FD_{x_0}[X, X^*|t_0](\xi) = |P(X = x_0|t_0) - P(X^{*} = x_0|t_0)|$. 
% }

% \sheng{
% For a $t_0$, the Fourier distance at a fixed pixel intensity $x_0$ is defined as $FD_{x_0}[X, X^*|t_0](\xi)$. 
% %
% By combining the probability of $x_0$ conditioned on $t_0$, we define a distance for all $x_0$ as $\sum_{x_0} P(x_0|t_0) FD_{x_0}[X, X^*|t_0](\xi)$. 
% %
% Then the distance for all $t_0$ can be formulated as 
% $$\sum_{t_0} P(t_0)\sum_{x_0}FD_{x_0}[X, X^*|t_0](\xi).$$
% %
% The distance can be viewed as the average Fourier distance among all $x_0$ and $t_0$. 
% %
% As there are two methods involving in computing the Fourier distance, we consider the conditional probability based on the ground truth as $P(x_0|t_0) = P(X_{gt}=x_0|t_0)$.
% %
% By combining all 
% If we want to sum these distances up, for each $FD_{x_0}[X, X^*|t_0](\xi)$, we need to multiply a weight $P(t_0)$, which represents the probability $t_0$ appears. Then the new Fourier distance becomes $\sum_{t_0} P(t_0)FD_{x_0}[X, X^*|t_0](\xi)$.
% %

% At each $t_0$, all $x_0$ should be treated equally. We directly average the distance at each $x_0$.
% $$\sum_{t_0} P(t_0)\sum_{x_0}FD_{x_0}[X, X^*|t_0](\xi)$$
% For computation, not all $x_0$ should be treated equally. The limited size of samples leads to the inaccuracy of distance at low probability area. Thus, we just consider a set of $x_0$. According to our grouping method, the similar inputs group together. Thus, the prediction output should be concentrated on some pixel intensity. Both of prediction probability distribution and ground truth probability distribution should be high at these pixel intensity. For example, the pixel intensity could be the average value of input patch. Therefore, at each $t_0$, we only consider the pixel intensity $x_0$ in a set, which has the high probability on both prediction distribution and ground truth distribution. For easier computation, we select the one that has the largest distance among the set. Therefore, the new Fourier distance should be like:
% $$\sum_{t_0} \sup_{x_0 \in A}P(t_0)FD_{x_0}[X, X^*|t_0](\xi)$$

% $A$ is the set that both $P(X = x_0|t_0)$ and $P(X^* = x_0|t_0)$ are high. 

% At this condition, we need to compute the set $A$ for each $t_0$. It is hard to compute and evaluate whether the probability is high. In addition, it is reasonable to believe that the distance should be low at the pixel intensity that prediction distribution probability or the ground truth distribution probability is low. Also, we could believe that the pixel intensity which gets largest distance is located at the set $A$. Therefore, we no longer need to compute the set $A$. Instead, we just need to find the largest distance among for all possible $x_0$. The new distance is 
% $$\sum_{t_0}  \sup_{x_0 \in \{0, 1, ..., 255\}}P(t_0)FD_{x_0}[X, X^*|t_0](\xi)$$

% We could find that 
% $$\sum_{t_0} \sup_{x_0 \in \{0, 1, ..., 255\}} P(t_0)FD_{x_0}[X, X^*|t_0](\xi) = \sum_{t_0}P(t_0)\sup_{x_0 \in \{0, 1, ..., 255\}}|P(X = x_0|t_0) - P(X^{*} = x_0|t_0)|$$
% }

% % \zhe{
% % $$\sum_{t_0} FD_{x_{0}}(X^{Est}, X^{Gt}| \xi\vec{k}\cdot\vec{I}_{n}) \quad != FD_{x_{0}}(X^{Est}, X^{Gt})$$
% % }

% In this case, we could define the Fourier distance as:

% $$FD_{x_0}[X, X^*](\xi) = \frac{1}{N} \left|\sum_{n}\mathbbm{1}(X_n = x_0)e^{-i\xi\vec{k}\cdot\vec{I_{n}}} - \sum_{n}\mathbbm{1}(X^*_n = x_0)e^{-i\xi\vec{k}\cdot\vec{I_{n}}} \right|$$


% The L2 distance is defined as 
% $$L_{2}(X, X^{*})  = \sum_{I}||X - X^{*}||^{2}_{2}$$

% We use the total variation distance\cite{gulrajani2017improved} as distribution distance. Thus, the distance is defined as 
% $$TV(X, X^*) = TV(D_X, D_{X^*}) = \sup_{\gamma \in \{0,..,255\}} |D_X(\gamma) - D_{X^{*}}(\gamma)|$$

% For a fix $t_0 = \vec{k}\cdot\vec{I}$

% $$TV(X, X^{*}|\vec{k}\cdot\vec{I} = t_0) = \sup_{\gamma \in \{0,..,255\}} |D_{X|t_0}(\gamma) - D_{X^{*}|t_0}(\gamma)|$$

% % \zhe{
% % $$t0 = \{0,1\}, and t0=0 -> D(Est) (0.9,0.1), t0=1 -> (0.1,0.9)$$
% % }

% Then we will point out what is the relaxation for easier understanding the relationship between these distances. First, we just consider one part of input $I$ because we divide the whole input set into two parts. One part is $\vec{k}\cdot\vec{I} = t_0$, while the other part is $\vec{k}\cdot\vec{I} \ne t_{0}$. If we get the relationship at each $t_{0}$, we could get the relationship at whole set. Second, for Fourier distance, we fix a frequency $\xi$, because the distribution measurements have no relation with frequency. 

% Under this definition, we want to prove that, for fix input $\vec{k}\cdot\vec{I} = t_0$ and frequency $\xi$. $X_{1}, X_{2}$ are predictions from two different models. $\forall x_{0}$, if $FD_{x_{0}}[X, X^*|\vec{k}\cdot\vec{I}](\xi)$ follows, $FD_{x_{0}}[X_{1}, X^{*}|\vec{k}\cdot\vec{I}] < FD_{x_{0}}[X_{2}, X^{*}|\vec{k}\cdot\vec{I}](\xi)$ , then we have the conclusion that $TV(X_{1}, X^{*}|\vec{k}\cdot\vec{I}) < TV(X_{2}, X^{*}|\vec{k}\cdot\vec{I})$. 


% \begin{proof}
%     For a fix input $t_0$ and frequency $\xi$, the magnitude of $\left|e^{-i\vec{k}\cdot\vec{I}}\right|$ is fixed. The Fourier distance is equal to the distribution distance at each $x_{0}$. 
    
%     $$FD_{x_0}[X, X^{*}|\vec{k}\cdot\vec{I}] = \left|P(X = x_0|\vec{k}\cdot\vec{I}) - P(X^{*} = x_0|\vec{k}\cdot\vec{I})\right|$$
    
%     We can find $x'$ satisfies  $$\sup_{\gamma \in \{0,..,255\}}|D_{X_{1}|\vec{k}\cdot\vec{I}}(\gamma) - D_{X^{*}|\vec{k}\cdot\vec{I}}(\gamma)| = |P(X_{1} = x'|\vec{k}\cdot\vec{I}) - P(X^{Gt} = x'|\vec{k}\cdot\vec{I})|$$ Then we can get 
%     \begin{align*}
%         & TV(X_{1}, X^{*}|\vec{k}\cdot\vec{I}) = \sup_{\gamma\in \{0,...,255\}}|D_{X_{1}|\vec{k}\cdot\vec{I}}(\gamma) - D_{X^{*}|\vec{k}\cdot\vec{I}}(\gamma)| = \\
%         & |P(X_{1} = x'|\vec{k}\cdot\vec{I}) - P(X^{*} = x'|\vec{k}\cdot\vec{I})| < |P(X_{2} = x'|\vec{k}\cdot\vec{I}) - P(X^{Gt} = x'|\vec{k}\cdot\vec{I})| \\
%         &  < \sup_{\gamma\in \{0,...,255\}}|D_{X_{2}|\vec{k}\cdot\vec{I}}(\gamma) - D_{X^{*}|\vec{k}\cdot\vec{I}}(\gamma)| = TV(X_{2}, X^{*}|\vec{k}\cdot\vec{I}) \\
%     \end{align*}

% \end{proof}


% \zhe{
% Once this is done, think about how to remove the $\xi\vec{k}\cdot\vec{I}_{n}$ condition. In other words, under what definition of $FD(X^{Est}, X^{Gt})$, we can derive $TV(X_{1}, X^{Gt}) < TV(X_{2}, X^{Gt})$ (or other forms of distribution distance) when $FD(X^{Est}_1, X^{Gt}) < FD(X^{Est}_2, X^{Gt})$ holds.



% After that, the next step will be
% \begin{itemize}
%     \item One-dimension $X$ (a looser case), treat $X$ as a pixel
%     \item High-dimension $X$ (a stricter case), treat $X$ as an image patch
% \end{itemize}
% }

% We remove the condition $\vec{k}\cdot\vec{I}$ and for a frequency $\xi$.
% The Fourier distance is 
% \begin{align*}
%     FD_{x_0}[X, X^{*}](\xi) &=  \left|F_{x_{0}}[X](\xi) - F_{x_{0}}[X^{*}](\xi) \right| \\
%     &=\frac{1}{N}\left( \left| \sum_{n} \mathbbm{1}(X = x_{0}) e^{-i\xi\vec{k}\cdot\vec{I_n}} - \sum_{n}\mathbbm{1}(X^{*} = x_{0}) e^{-i\xi\vec{k}\cdot\vec{I_n}} \right| \right) \\
%     &= \frac{1}{N}\left| \sum_{t_0}\left(\sum_{n, s.t.,\vec{k}\cdot\vec{I_n}=t_0}(\mathbbm{1}(X = x_{0}) e^{-i\xi\vec{k}\cdot\vec{I_n}})-\sum_{I, s.t.,\xi\vec{k}\cdot\vec{I}_{n}}\mathbbm{1}(X^{*} = x_{0}) e^{-i\xi\vec{k}\cdot\vec{I_n}} \right)\right| \\
%     &= \frac{1}{N}\left|\sum_{t_0}\left(e^{-it_0\xi} \sum_{I, s.t.,\vec{k}\cdot\vec{I}_{n} = t_0}\left(\mathbbm{1}(X = x_{0}) - \mathbbm{1}(X^{*} = x_{0})  \right)\right) \right| \\
%     &=\left|\sum_{t_0}e^{-it_0\xi}\left(P(X = x_0, t_0) - P(X^{*} = x_0, t_0) \right)  \right| \\
%     &=\left|\sum_{t_0}e^{-it_0\xi}P(t_0)\left(P(X = x_0|t_0) - P(X^{*} = x_0| t_0) \right) \right| \\ 
%     &= \left|E_{t_0}\left[e^{-it_0\xi}\left(P(X = x_0|t_0) - P(X^{*} = x_0| t_0) \right) \right]\right|
% \end{align*}


% The Total Variation distance is 
% \begin{align*}
%     TV(X, X^{*}) &= \sup_{x_0 \in \{0,..,255\}}|D_{X}(x_0) - D_{X^{*}}(x_0)| \\ 
%     &= \max_{x_0 \in \{0,..,255\}}|P(X = x_0) - P(X^{*} = x_0)| \\
%     &= \max_{x_0 \in \{0,..,255\}}\left|\sum_{t_0}(P(t_0)P(X = x_0|t_0)) - \sum_{t_0}(P(t_0)P(X^{*} = x_0|t_0)) \right| \\
%     &= \max_{x_0 \in \{0,..,255\}}\left|\sum_{t_0}P(t_0)\left( P(X = x_0|t_0) - P(X^{*} = x_0|t_0)\right) \right| \\
%     &= \max_{x_0 \in \{0,..,255\}}\left|E_{t_0}\left[P(X = x_0|t_0) - P(X^{*} = x_0|t_0) \right] \right| 
% \end{align*}

% \zhe{The ideal case is to design a metric based on $TV(X, X^{*}|I)$ for all the input $I$, e.g., $\sum_I TV(X, X^{*}|I)$.}

% Here, we need to re-design the Fourier distance. Before this step, we first want to show correctness of distribution distance. Here, the distribution distance is not the output distribution of pixel intensity on whole dataset. It is a combination of distribution of pixel intensity condition on low resolution input. For simplicity, we use TV distribution distance as example.

% In this paper, we believe that at each pixel point, the high resolution output is not only a scalar, but a distribution. The pixel intensity at given high resolution image is one of the possible value according to the input image patch. Therefore, the mapping from input low resolution image patch to high resolution pixel intensity is a one to many mapping. To get the distribution of output pixel intensity, we need to sample the same inputs. However, due to limitation of sample size, it is hard to sample the same inputs in all image patches. To make it simpler, we take a subset of low resolution inputs which has same properties to replace a single input to get the output distribution. 

% Therefore, to get the distribution of output high resolution images, we need to group the input low resolution images. One of the grouping method is to project input low resolution input to one dimension, which has more similar samples to get output distribution. In this section, we project the input low resolution image on the direction of first principle component. And the number of group is 200. As it shows, the $t = \vec{k}\cdot\vec{I}$ is the one dimension projection of inputs. The combination of all distribution which condition on same $t = t_0$ is the weight sum by the probability $P(t = t_0)$. 

% \begin{align*}
%     \sum_{t_0}P(t_0)TV(X_n, X^*_n|t_0) &= \sum_{t_0} P(t=t_0)TV(X, X^*|t_0) \\
%     &=\sum_{t_0} P(t=t_0)\sup_{x_0 \in \{0,1,..,255\}}\left| P(X=x_0|t_0) - P(X^*=x_0|t_0)\right| \\
%     &= \sum_{t}P(t=t_0)FD_{x', s.t. \text{argmax}|P(X=x'|t_0) - P(X^*=x'|t_0)|}[X, X^*|t_0](\xi)
% \end{align*}





% \sheng{
% My question is :
% After considering different distribution distance, both of these distances consider the sample $X_0 \in \{0,255\}$ with same weight. In Fourier Distance $F_{X_0}(X) = \sum_I P(X = X_0)e^{-ikI}$. For different $X_0$, It has different weight. 

% What we have is $\left|\sum_i a_i*x_{1i} \right| \le \left| \sum_i a_i*x_{1i} \right|$, and we want to get $\left|\sum_i b_i * x_{1i} \right| \le \left| \sum_i b_i*x_{1i} \right|$. It does not work form LHS to RHS or RHS to LHS. 

% }

% \sheng{\textbf{}
% $$TV(X^{Est}, X^{Gt}) = \sup_{\gamma \in \{0,..,255\}}\left|D(X^{Est})(\gamma) - D(X^{Gt})(\gamma))\right| = \max_{x_0 \in \{0,..,255\}}|P(X^{Est} = x_0) - P(X^{Gt} = x_0)|$$

% $$KL(X^{Est}, X^{Gt}) = \sum_{\gamma \in \{0,..,255\}} D(X^{Est})(\gamma)\log\left(\frac{D(X^{Gt})(\gamma)}{D(X^{Est})(\gamma)}\right))  = \sum_{x_0\in \{0,..,255\}}P(X^{Est} = x_0)\log\left(\frac{P(X^{Gt} = x_0)}{P(X^{Est} = x_0)}\right)$$
% $$Wass(D(X^{Est}), D(X^{Gt})) = \sup_{f, |f|_{Lip} \le 1}\left|\int_{\gamma\in \{0,..,255\}} f(\gamma)d(D(X^{Est})(\gamma)- D(X^{Gt})(\gamma))\right|$$
% }


% \sheng{
% Back to the original definition of $F_{x_0}(X) = \frac{1}{N}\sum_{I}\mathbbm{1}(X = x_0, I)e^{-ikI}$. From sample point, compared with $P(X = x_0) = \frac{1}{N}\sum_{I}\mathbbm{1}(X = x_0, I)$, for each input sample $I$, it has a weight $e^{-ikI}$. Therefore, one of my idea is to remove the impact of $e^{-ikI}$. Forcing $kI = constant$ is a straightforward idea, seeing the explanation below. For different distribution measurement, there are different solution. For the distribution which must consider each $P(X = X_0)$. We must establish a equation between $F_{X_0}$ and $P(X = X_0)$. Fixed $I$ and $k$ satisfies this requirement. For the distribution measurement that consider the sum of all $P(X = X_0)$, we could consider add a weight to each $X_0$, which originally is uniform distribution, such that removing the impact of $e^{-ikI}$.  
% }

% \sheng{
% From The definition of all probability measurement, we could find that  
% We want to find a $\vec{k}$ that $\forall I, \vec{k}I = b$, $b$ is a constant here. Consider a input matrix $M$. The row is the number of input data, and the column is the dimension of input data. We want to find a $\vec{k}$ that $M\vec{k} = b\vec{1}$. Thus, $\forall I, Ik = b$. 
% $$F_{X_{0}}(X) = \frac{1}{N}\left|\sum_{I}\mathbbm{1}(X = X_{0}) e^{-iIk} \right| = \frac{1}{N}\left|\sum_{I}\mathbbm{1}(X = X_{0}) e^{-ib} \right| = P(X = X_0)$$
% }

% \sheng{
%     $$F_{x_{0}}(X) = \frac{1}{N}\sum_{I}\mathbbm{1}(X = x_{0}, I) e^{-ikI} $$
% }

% \section{User Study}
% In super resolution area, the most common evaluation metric are PSNR and SSIM. However, both of these evaluation metric are not close to the result by human vision, In this case, We want to design a new evaluation metric whose result is close to the result by human vision. 

% To show that our evaluation metric is close the the result by human vision, we need to explore the correlation between the ranking result by human vision and our evaluation metric on different super resolution methods. If the ranking result by our evaluation metric has high correlation with ranking result by human result, it shows that our evaluation reflects human vision well. \sheng{
% To get the correlation of two ranking, we use Spearman's rank correlation coefficient and Pearson correlation coefficient to measure the monotonic and linear relationship of two rank result, corresponding to the rank from designed evaluation metric and human vision ranking result. Thus, we collect the ranking result from common evalutaion metric such as PSNR and SSIM, as well as our evaluation metric.
% }

% Therefore, we need to design a user study to explore the human's ranking on different super resolution methods. A straightforward idea is to show all super resolution methods on a image to rank. However, this approach would be not accurate when some methods get similar result. Thus, we take pair comparison strategy for user study. We mainly have two problems on the survey. First, how to select appropriate image patch for the survey? Second, how to evaluate one method which is better than the other?

% In recent super resolution methods, the full size view of a image is not distinguishable on different methods. Human could find subtle difference unless on small image patch such as $200 \times 200$. To better showing the difference between different methods, we assume the pixel distribution at each pixel is a Gaussian distribution. And we calculate the average standard deviation/mean in a image patch. We divide standard deviation by mean to remove the affect of pixel value itself. In addition, some methods in a image patch could be regarded as outlier which is out of $3\sigma$. Besides, we will not put the ground truth high resolution image anywhere in our survey because it will mislead user to select method which is close to ground truth. Overall, we select the image patch whose size is $200 \times 200$ and has highest average standard deviation/mean value in a image. 

% After given a image patch and pair comparison strategy, we need to compare the result upscaled from low resolution image by two different super resolution methods. We could directly ask the user to choose which one is better. However, the evaluation result might not be consistent for this abstract question because the user might also be confused about the criterion of a "good" super resolution result. Therefore, we separate this abstract question into several specific questions. First, as a super resolution problem, the primary goal is to get sharp image from blur and smooth low resolution image. In this process, some methods still generate blur image. Others might generate image with large noise or ringing. Naturally, sharpness is one of the criterion evaluation. Second, because we get high resolution image from low resolution image, information from low resolution image is not enough. Thus, some methods might generate image which is fake or unnatural from human's common sense. For example, the change of shape, such as a straight line is no longer straight, could be considered as a fake content in high resolution image. The shadow and stereoscopy could also influence user's judgment. Therefore, authenticity could also be one of the criterion for evaluation. In conclusion, we will set two questions from sharpness and authenticity aspects for user to evaluate different super resolution methods.

% All in all, we take pair comparison strategy, select appropriate image patch and set reasonable questions for user study. After collecting data from user study, we could get the user's ranking or preference on different super resolution methods. We explore the correlation between human's result with our evaluation metric and other popular evaluation metric in this area. We want that our evaluation metric stands out against other evaluation metrics. 
% \zhe{How to evaluate the correlation? What methods to use? If using those methods, are there any other information needed? Describe and think more in details.}

% \subsection{User feedback}
% \begin{itemize}
%     \item The first expression of user on different super resolution methods is how sharp the image could be generated. If there is not any suggestion about authenticity, they will only consider the sharpness.
%     \item The users' expression on authenticity of a image generated by a super resolution method is mainly on the shape of the object. For example, a fake content might be a non-straight line where should be a straight line. They also focus on the shadow of a object which reflects the stereoscopy of the image. 
%     \item The user mention that some area should be blur such as the background of a image. If a super resolution method makes it sharper, the method is not a good method. 
% \end{itemize}

% \section{Related Work}
% \subsection{Fourier Transform on neural network}
% \subsection{metrics}
% \subsubsection{full reference metrics}
% \subsection{Different pairwise comparison method}
% The problem setting is that we have $N$ methods, the counting matrix $C_{ij}$ represnets the number that method $i$ wins method $j$, where $\{i, j\} \in N$. The target is to rank $N$ methods by the counting matrix $C$.
% A straightforward method to covert pairwise comparison to to an overall comparison by sorting the fraction of the number of times $i$ wins. However, it could be affected by the missing data and overfitting.  

% The probabilistic model for pairwise comparison is a better choice. The target is to get a probability matrix $M_{ij}$, which $M_{ij}$ is the probability that $i$ wins $j$. 

% The Thurstone’s Model assumes that the probability of a human selecting a method $I$ follows Gaussian distribution. Thus, for method $I$ and $J$, the distributions are $I \sim \mathcal{N}(\mu_i, \sigma_i)$, $J \sim \mathcal{N}(\mu_j, \sigma_j)$. In this case, the probability that $M_{ij} = P(I>J) = P(I-J>0)$. It is the subtraction of two Gaussian distribution, which is $I-J \sim \mathcal{N}(\mu_i-\mu_j, \sqrt{\sigma_i^2 + \sigma_j^2 - 2\sigma_i\sigma_j\rho_{ij}})$. We rewrite is as $I-J \sim \mathcal{N}(\mu_{ij}, \sigma_{ij})$. Also $p(i > j | \mu) = M_{ij} = \Phi (\mu_i - \mu_j)$ for $\sigma_i^2 = \sigma_j^2 = 0.5, \rho_{ij} = 0$. 

% The Bradley-Terry model remove the assumption that the distribution is Gaussian. And it changes the function $\Phi$ to logistic function. $M_{ij} = \Phi(\mu_i - \mu_j) = \frac{1}{1+e^{\mu_i-\mu_j}}$. $\mu_i$ and $\mu_j$ is no longer the mean of Gaussian distribution.

% The Elo rating method is close to Bradeley-Terry method. It changes the fuction to $\Phi = \frac{1}{1+10^{\frac{\mu_i-\mu_j}{400}}}$. The Glicko method improve the Elo rating system by a Bayesian framework. The TrueSkill system is an online rating system which consider the multi-player game.  

% Both those models could be accounted for a Bayesian model and get latent result result by the maximum likelihood estimation. $P(C|\mu) = \Pi_{ij}[\Phi(\mu_i - \mu_j)]^{C_{ij}} \cong \sum_{ij}C_{ij}\log(\Phi(\mu_i - \mu_j))$ . Thus, the question transfer to a optimization problem:
% $$ \underset{\mu}{\text{argmax}} \sum_{ij}C_{ij}\log(\Phi(\mu_i - \mu_j))$$
% $$\text{subject to} \sum_{i} \mu_i = \text{constant}$$

% \section{Fourier Distance Experiment}
% In this section, I will design a Fourier distance metric method from both theory and experiment. 

% First, the basic formulation for Fourier transform for sample and Fourier distance are $$F_{x_0}[X](\xi) = \frac{1}{N}\sum_{n}\mathbbm{1}(X_n = x_0) e^{-i\xi\vec{k}\cdot\vec{I_{n}}}$$
% $$F_{x_0}[X|\vec{k}\vec{I}](\xi) = \frac{1}{N}\sum_{n}\mathbbm{1}(X_n = x_0|\vec{k}\vec{I}) e^{-i\xi\vec{k}\cdot\vec{I_{n}}}$$
% $$\left|F[X](\xi)\right| = \frac{1}{N}\left|\sum_{x_0}P(x_0)\sum_{n}\mathbbm{1}(X_n = x_0) e^{-i\xi\vec{k}\cdot\vec{I_{n}}} \right|$$
% $$FD_{x_0}[X, X^*](\xi) = \frac{1}{N} \left|\sum_{n}\mathbbm{1}(X_n = x_0)e^{-i\xi\vec{k}\cdot\vec{I_{n}}} - \sum_{n}\mathbbm{1}(X^*_n = x_0)e^{-i\xi\vec{k}\cdot\vec{I_{n}}} \right|$$
% $$FD[X, X^*](\xi) = \frac{1}{N}\sum_{x_0}P(x_0) \left|\sum_{n}\mathbbm{1}(X_n = x_0)e^{-i\xi\vec{k}\cdot\vec{I_{n}}} - \sum_{n}\mathbbm{1}(X^*_n = x_0)e^{-i\xi\vec{k}\cdot\vec{I_{n}}} \right|$$
% In this equation, we need to fix the parameters frequency $\xi$, pixel intensity $x_0$, direction of $\vec{k}$ and sampling method. 

% \subsection{Pixel Intensity $x_0$}
% $$F[X](\xi) = \sum_{x_0} F_{x_0}[X](\xi) = \frac{1}{N}\sum_{x_0}\sum_{n}\mathbbm{1}(X_n = x_0) e^{-i\xi\vec{k}\cdot\vec{I_{n}}} = \frac{1}{N} \sum_{n}e^{-i\xi\vec{k}\cdot\vec{I_{n}}}$$
% \subsection{Sampling Method}
% \subsection{Direction of $\vec{k}$}
% To reduce the dimension of input $I$ to one dimension, there are two possible choice for direction of $\vec{k}$
% \subsection{Frequency}



% \section{Survey}
% \subsection{Image Area Selection}
% In this paper, we evaluate different super resolution method on DIV2K test dataset. For human study, the full size view of image is not distinguishable. Human could find the subtle difference until the image patch size is small, such as 200 $\times$ 200 in our setting. We select one image area on each test image. This area should be the best to present the difference of different methods. Therefore, we first assume that for each pixel location, the distribution of pixel intensity is Gaussian distribution. 



